Neutrino properties from the laboratory and the cosmos

Neutrinos are amongst the most abundant particles in the universe. The fact that they are massive particles proves that the Standard Model is an incomplete theory and needs to be extended. This thesis focuses on the study of neutrino properties from the available data from laboratory experiments and cosmological observations. It also presents sensitivity studies for future neutrino experiments. The first part covers the status of the determination of the oscillation parameters in the three-neutrino framework, the mass ordering and the absolute mass scale. A second part is devoted to other neutrino properties predicted in neutrino mass models. The topics covered include the study of spin-flavour precession in solar neutrinos from non-zero neutrino magnetic moments, the prospects for neutrino non-standard interactions with quarks from the solar sector and the expected limits on CPT violation from a separate analysis of neutrino and antineutrino data. Regarding cosmology, the impact of non-standard interactions with electrons and a non-unitary three-neutrino mixing matrix in the process of neutrino decoupling are addressed. Finally, a third part explores possible connections between dark matter and neutrinos. The existence of dark matter has been proven indirectly via its gravitational effects. This thesis presents two studies that explore how neutrinos could probe the fraction of dark matter that could exist in the form of primordial black holes and the experimental signatures expected from a hypothetical coupling between neutrinos and an ultralight scalar dark matter candidate.

==> intro.tex <==
Blablabla
